Shape Your Ground: Refining Road Surfaces Beyond Planar Representations

Road surface reconstruction from aerial images is fundamental for autonomous driving, urban planning, and virtual simulation, where smoothness, compactness, and accuracy are critical quality factors. Existing reconstruction methods often produce artifacts and inconsistencies that limit usability, while downstream tasks have a tendency to represent roads as planes for simplicity but at the cost of accuracy. We introduce FlexRoad, the first framework to directly address road surface smoothing by fitting Non-Uniform Rational B-Splines (NURBS) surfaces to 3D road points obtained from photogrammetric reconstructions or geodata providers. Our method at its core utilizes the Elevation-Constrained Spatial Road Clustering (ECSRC) algorithm for robust anomaly correction, significantly reducing surface roughness and fitting errors. To facilitate quantitative comparison between road surface reconstruction methods, we present GeoRoad Dataset (GeRoD), a diverse collection of road surface and terrain profiles derived from openly accessible geodata. Experiments on GeRoD and the photogrammetry-based DeepScenario Open 3D Dataset (DSC3D) demonstrate that FlexRoad considerably surpasses commonly used road surface representations across various metrics while being insensitive to various input sources, terrains, and noise types. By performing ablation studies, we identify the key role of each component towards high-quality reconstruction performance, making FlexRoad a generic method for realistic road surface modeling.

==> tables/dsc_full.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

% TODO: merge to the prev table
\begin{table}[h]
  \centering
  \caption{\textbf{Road Fitting Results on DeepScenario Datasets.} The results for $\mathcal{L}_2$ and Mean Absolute Deviation (MAD) are presented in meters and degrees, respectively. The primary input for \ourmethod is $\mathbf{R}^{DSM}$, from which $\mathbf{R}^{road+}$ is automatically extracted following our pipeline. The inputs listed here pertain to the terrain support. The term DS refers to the dynamic sampling approach used when creating the mesh.}
  \label{tab:results_on_dsc}
    \begin{tabular}{P{3.2cm} | c | c | c | c | c | c | P{0.8cm}}
      \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Input} & \multirow{2}{*}{\acs{FILTER}} & \multicolumn{2}{c|}{$\mathcal{L}_2$} & \multicolumn{2}{c|}{\ac{MAD}} & \multirow{2}{*}{$T$} \\
        \cmidrule(lr){4-7}
          & &  & Road & Terrain & Road & Terrain & \\
        \midrule
         \multirow{2}{*}{Plane} & $\mathbf{R}^{DSM}$ & \xmark & 1.163 & 2.727 & 0 & 0 & 2 \\
         & $\mathbf{R}^{DTM}_{V}$ & \xmark & 1.251 & 2.002 & 0 & 0 & 2 \\
        \midrule
    
        \multirow{6}{*}{Delaunay \cite{delaunay_1934}} & $\mathbf{R}^{DSM}$ & \xmark & 0.195 & 15.411 & 7.185 & 15.78 & 45K \\
          & $\mathbf{R}^{DTM}_{S}$ & \xmark & 0.308 & 1.087 & 4.577 & 2.079 & 139K \\
          & $\mathbf{R}^{DTM}_{S}$ & \cmark & 0.288 & 2.875 & 5.201 & 1.89 & 139K \\
          & $\mathbf{R}^{DTM}_{V}$ & \xmark & 0.308 & 1.087 & 4.577 & 2.079 & 139K \\
          & $\mathbf{R}^{DTM}_{V}$ & \cmark & 0.221 & 0.971 & 3.131 & 0.701 & 139K\\
        \cmidrule(lr){1-8}
        \multirow{2}{*}{\ourmethod~{\scriptsize (Ours)}} & $\mathbf{R}^{DSM}$ & \cmark & 0.104 & 3.511 & 0.576 & 0.861 & 185K\\
          & $\mathbf{R}^{DTM}_{V}$ & \cmark & 0.106 & 0.528 & 0.457 & 0.569 & 185K\\
        \cmidrule(lr){1-8}
        \multirow{2}{*}{\ourmethod + DS~{\scriptsize (Ours)}} & $\mathbf{R}^{DSM}$ & \cmark & 0.104 & 3.508 & 0.547 & 2.533 & 59K\\
          & $\mathbf{R}^{DTM}_{V}$ & \cmark & 0.106 & 0.524 & 0.43 & 1.927 & 59K\\
        \bottomrule
    \end{tabular}
  \vspace*{-1\baselineskip}
\end{table}

==> tables/geobasis_full.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}


\begin{table}[h]
    \centering
    \scriptsize
    \caption{\textbf{Road fitting results on \ac{GeoRoad} Datasets.} The results for $\mathcal{L}_2$ and \acs{MAD} are presented in meters and degrees, respectively. The primary input for \ourmethod is $\mathbf{R}^{DSM}$, from which $\mathbf{R}^{road+}$ is automatically extracted following our pipeline. The inputs of \ourmethod listed here pertain to the terrain support. The term GF refers to the Gaussian Filtering used to smoothen the surface.}
    \label{tab:results_on_geobasisroad}
    \footnotesize
        \begin{tabular}{P{1cm} | c | c | c | c | c | c | c | P{0.8cm}}
        \toprule
            \multirow{2}{*}{\makecell{Tile\\Size}} & \multirow{2}{*}{Method} & \multirow{2}{*}{Input} & \multirow{2}{*}{\acs{FILTER}} & \multicolumn{2}{c|}{$\mathcal{L}_2$ $\downarrow$} & \multicolumn{2}{c|}{\acs{MAD} $\downarrow$} & \multirow{2}{*}{$T \downarrow$} \\    
            \cmidrule(lr){5-8}
             & & & & Road & Terrain & Road & Terrain & \\    
        \midrule
            \multirow{14}{*}{\adjustbox{angle=90,valign=m}{$250\text{m} \times 250\text{m}$}} 
            & \multirow{2}{*}{Plane} & $\mathbf{R}^{DSM}$ & \cmark & 2.05 & 2.343 & 0 & 0 & 2\\
            & & $\mathbf{R}^{DTM}_{GT}$ & \xmark & 1.813 & 2.013 & 0 & 0 & 2\\
        \cmidrule(lr){2-9}
            & \multirow{6}{*}{\acs{RGT}} & $\mathbf{R}^{DSM}$ & \xmark & 0.415 & 1.773 & 15.55 & 22.191 & 124K\\
            & & $\mathbf{R}^{DTM}_{GT}$ & \xmark & 0 & 0 & 2.141 & 2.652 & 123K\\
            & & $\mathbf{R}^{DTM}_{S}$ & \xmark & 0.414 & 1.326 & 15.621 & 8.445 & 124K\\
            & & $\mathbf{R}^{DTM}_{S}$ & \cmark & 0.965 & 0.92 & 3.385 & 2.972 & 124K\\
            & & $\mathbf{R}^{DTM}_{V}$ & \xmark & 0.415 & 0.525 & 15.32 & 3.521 & 124K\\
            & & $\mathbf{R}^{DTM}_{V}$ & \cmark & 1.124 & 1.364 & 2.911 & 0.972 & 124K\\
        \cmidrule(lr){2-9}
            & \multirow{2}{*}{GF + \acs{RGT}} & $\mathbf{R}^{DSM}$ & \xmark & 4.33 & 5.08 & 0.108 & 0.108 & 123K\\
            & & $\mathbf{R}^{DTM}_{GT}$ & \xmark & 0.587 & 0.473 & 0.03 & 0.029 & 123K\\
        \cmidrule(lr){2-9}
            & \multirow{3}{*}{{${\text{\ourmethod}}_{\text{\acs{RGT}}}$~{\scriptsize (Ours)}}} & $\mathbf{R}^{DSM}$ & \cmark & 0.586 & 2.984 & 0.577 & 0.986 & 123K\\
            & & $\mathbf{R}^{DTM}_{GT}$ & \cmark & 0.181 & 0.321 & 0.391 & 0.588 & 123K\\
            & & $\mathbf{R}^{DTM}_{V}$ & \cmark & 0.615 & 1.48 & 0.573 & 0.619 & 122K\\
        \cmidrule(lr){2-9}
            & \multirow{3}{*}{${\text{\ourmethod}}_{\text{\acs{TIN}}}$~{\scriptsize (Ours)}} & $\mathbf{R}^{DSM}$ & \cmark & 0.584 & 2.941 & 1.081 & 3.635 & 33K\\
            & & $\mathbf{R}^{DTM}_{GT}$ & \xmark & 0.18 & 0.313 & 0.897 & 2.846 & 33K\\
            & & $\mathbf{R}^{DTM}_{V}$ & \cmark & 0.604 & 1.449 & 1.107 & 3.062 & 33K\\ %TODO: check why road performance got worse in DS (smoothness)
        \midrule
            \multirow{13}{*}{\adjustbox{angle=90,valign=m}{$500\text{m} \times 500\text{m}$}} 
            & \multirow{2}{*}{Plane} & $\mathbf{R}^{DSM}$ & \cmark & 3.022 & 3.855 & 0 & 0 & 2\\
            & & $\mathbf{R}^{DTM}_{GT}$ & \xmark & 3.578 & 6.457 & 0 & 0 & 2 \\
        \cmidrule(lr){2-9}
            & \multirow{6}{*}{\acs{RGT}} & $\mathbf{R}^{DSM}$ & \xmark & 0.407 & 1.77 & 15.593 & 22.334 & 498K\\
            & & $\mathbf{R}^{DTM}_{GT}$ & \xmark & 0 & 0 & 2.095 & 2.665 & 496K\\
            & & $\mathbf{R}^{DTM}_{S}$ & \xmark & 17.338 & 16.892 & 14.572 & 8.631 & 873K\\ % Here some locations show highway roads wihout few to no building. These DSM to DTM converter will probaly fail, e.g. 402000_5757000, 409000_5759000
            & & $\mathbf{R}^{DTM}_{S}$ & \cmark & 0.406 & 1.173 & 3.532 & 3.086 & 499K\\
            & & $\mathbf{R}^{DTM}_{V}$ & \xmark & 0.408 & 0.496 & 15.305 & 3.323 & 498K\\
            & & $\mathbf{R}^{DTM}_{V}$ & \cmark & 18.032 & 17.371 & 2.458 & 1.092 & 872K\\
        \cmidrule(lr){2-9}
            & GF + \acs{RGT} & $\mathbf{R}^{DSM}$ & \xmark & 0.467 & 0.458 & 0.032 & 0.032 & 498K\\
        \cmidrule(lr){2-9}
            & \multirow{3}{*}{{${\text{\ourmethod}}_{\text{\acs{RGT}}}$~{\scriptsize (Ours)}}} & $\mathbf{R}^{DSM}$ & \cmark & 0.243 & 4.03 & 0.248 & 0.45 & 496K \\
            & & $\mathbf{R}^{DTM}_{GT}$ & \xmark & 0.071 & 0.599 & 0.199 & 0.283 & 496K\\
            & & $\mathbf{R}^{DTM}_{V}$ & \cmark & 0.423 & 1.954 & 0.235 & 0.298 & 494K\\
        \midrule
            \multirow{13}{*}{\adjustbox{angle=90,valign=m}{$1000\text{m} \times 1000\text{m}$}} 
            & \multirow{2}{*}{Plane} & $\mathbf{R}^{DSM}$ & \cmark & 3.715 & 5.53 & 0 & 0 & 2 \\
            & & $\mathbf{R}^{DTM}_{GT}$ & \xmark & 6.435 & 8.164 & 0 & 0 & 2 \\
        \cmidrule(lr){2-9}
            & \multirow{6}{*}{\acs{RGT}} & $\mathbf{R}^{DSM}$ & \xmark & 0.372 & 1.757 & 14.883 & 22.322 & 1.9M\\
            & & $\mathbf{R}^{DTM}_{GT}$ & \xmark & 0 & 0 & 2.011 & 2.672 & 1.9M\\
            & & $\mathbf{R}^{DTM}_{S}$ & \xmark & 0.37 & 1.338 & 14.873 & 8.409 & 1.9M\\
            & & $\mathbf{R}^{DTM}_{S}$ & \cmark & 0.142 & 1.987 & 3.616 & 3.066 & 1.9M\\
            & & $\mathbf{R}^{DTM}_{V}$ & \xmark & 0.373 &  0.473 & 14.588 & 3.345 & 1.9M\\
            & & $\mathbf{R}^{DTM}_{V}$ & \cmark & 0.5 & 2.457 & 3.114 & 1.019 & 1.9M\\
        \cmidrule(lr){2-9}
            & GF + \acs{RGT} & $\mathbf{R}^{DSM}$ & \xmark & 3.697 & 3.125 & 0.028 & 0.034 & 1.9M\\
        \cmidrule(lr){2-9}
            & \multirow{3}{*}{{${\text{\ourmethod}}_{\text{\acs{RGT}}}$~{\scriptsize (Ours)}}} & $\mathbf{R}^{DSM}$ & \cmark & 0.606 & 2.594 & 0.089 & 0.102 & 1.9M\\
            & & $\mathbf{R}^{DTM}_{GT}$ & \xmark & 0.114 & 1.034 & 0.08 & 0.102 & 1.9M\\
            & & $\mathbf{R}^{DTM}_{V}$ & \cmark & 0.221 & 2.422 & 0.082 & 0.096 & 1.9M\\
        \bottomrule
        \end{tabular}
    \vspace*{-1\baselineskip}
\end{table}

